Mining Closed Strict Episodes

Discovering patterns in a sequence is an important aspect of data mining. One popular choice of such patterns are episodes, patterns in sequential data describing events that often occur in the vicinity of each other. Episodes also enforce in which order the events are allowed to occur. In this work we introduce a technique for discovering closed episodes. Adopting existing approaches for discovering traditional patterns, such as closed itemsets, to episodes is not straightforward. First of all, we cannot define a unique closure based on frequency because an episode may have several closed superepisodes. Moreover, to define a closedness concept for episodes we need a subset relationship between episodes, which is not trivial to define. We approach these problems by introducing strict episodes. We argue that this class is general enough, and at the same time we are able to define a natural subset relationship within it and use it efficiently. In order to mine closed episodes we define an auxiliary closure operator. We show that this closure satisfies the needed properties so that we can use the existing framework for mining closed patterns. Discovering the true closed episodes can be done as a post-processing step. We combine these observations into an efficient mining algorithm and demonstrate empirically its performance in practice.

==> pics/Makefile <==
DOTSRCS = toy1.dot toy2.dot toy3.dot toy4.dot toy4a.dot toy5.dot toy6.dot \
	closure1.dot closure2.dot closure3.dot closure4.dot closure5.dot closure6.dot \
	join1_1.dot join1_2.dot join1_3.dot join1_4.dot join1_5.dot \
	join2_1.dot join2_2.dot join2_3.dot \
	test_1.dot test_2.dot test_3.dot test_4.dot \
	fail_1.dot fail_2.dot fail_3.dot
EPSES = $(DOTSRCS:.dot=.tex)



all : $(EPSES)

%.tex : %.dot
	dot2tex -t raw $*.dot | sed '1,25d; $d' | sed -e :a -e '$d;N;2,9ba' -e 'P;D' > $*.tex


==> pics/join2_1.tex <==
\pgfsetcolor{black}
  % Edge: c -> a
  \draw [->] (53.916bp,71.831bp) .. controls (49.939bp,63.877bp) and (45.185bp,54.369bp)  .. (36.207bp,36.413bp);
  % Edge: c -> b
  \draw [->] (72.084bp,71.831bp) .. controls (76.061bp,63.877bp) and (80.815bp,54.369bp)  .. (89.793bp,36.413bp);
  % Node: a
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (27bp,18bp) node {$a$};
\end{scope}
  % Node: c
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (63bp,90bp) node {$c$};
\end{scope}
  % Node: b
\begin{scope}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (99bp,18bp) node {$b$};
\end{scope}
%

